Computing discrete logarithm by interval-valued paradigm

Interval-valued computing is a relatively new computing paradigm. It uses finitely many interval segments over the unit interval in a computation as data structure. The satisfiability of Quantified Boolean formulae and other hard problems, like integer factorization, can be solved in an effective way by its massive parallelism. The discrete logarithm problem plays an important role in practice, there are cryptographical methods based on its computational hardness. In this paper we show that the discrete logarithm problem is computable by an interval-valued computing in a polynomial number of steps (within this paradigm).

==> eptcsdata.tex <==
\providecommand{\firstpage}{76}
\providecommand{\publicationstatus}{B. L\"owe, G. Winskel (Eds.):\\
Developments in Computational Models 2012 (DCM 2012)\\
EPTCS 143, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.143.7}{10.4204/EPTCS.143.7}}
\pdfoutput=1

